Turning an Urban Scene Video into a Cinemagraph

This paper proposes an algorithm that turns a regular video capturing urban scenes into a high-quality endless animation, known as a Cinemagraph. The creation of a Cinemagraph usually requires a static camera in a carefully configured scene. The task becomes challenging for a regular video with a moving camera and objects. Our approach first warps an input video into the viewpoint of a reference camera. Based on the warped video, we propose effective temporal analysis algorithms to detect regions with static geometry and dynamic appearance, where geometric modeling is reliable and visually attractive animations can be created. Lastly, the algorithm applies a sequence of video processing techniques to produce a Cinemagraph movie. We have tested the proposed approach on numerous challenging real scenes. To our knowledge, this work is the first to automatically generate Cinemagraph animations from regular movies in the wild.

==> classification.tex <==
\section{Random forest classifier}
\begin{table*}[t]
  \centering
  \begin{tabular}{|p{0.09\textwidth}|p{0.14\textwidth}|p{0.63\textwidth}|p{0.04\textwidth}|}
    \hline
    Category & Feature & description & Dim \\
    \hline
    \multirow{3}{*}{Appearance} & RGB mean & Mean RGB values. & 3\\ \cline{2-4}
    & RGB variance & Variances of RGB values.& 3\\ \cline{2-4}
    & LAB histogram & Histogram in LAB color space with 8 bins for each channel. & 24 \\
    \hline
    Gradient & BoW & Bag-of-words descriptors constructed by K-means clustering on HoG3D
    descriptor~\cite{klaser2008spatio} extracted from regular grid points. & 100\\
    \hline
    \multirow{5}{*}{Shape} & Area & Ratio of the 2D area against the area of the entire frame. & 1\\ \cline{2-4}
    & Convexity & Ratio of the 2D area against the area of its convex hull. & 1 \\ \cline{2-4}
    & Rectangleness & Ratio of the 2D area against the area of the minimum bounding box. & 1\\ \cline{2-4}
    & Aspect ratio & The aspect ratio of the minimum bounding box. & 1 \\ \cline{2-4}
    & Number of edges & The number of edges of an approximated 2D
    shape. The approximation error is set to 1\% of the smaller dimension of the frame. & 1\\
    \hline
    \multirow{2}{*}{Position} & Centroid & The position of the
    centroid of the segment. & 2\\ \cline{2-4}
    &Bounding box & Minimum/maximum x/y position, normalized by width
    and height. & 4\\
    \hline
  \end{tabular}
  \caption{The feature vector used for random forest.}
  \label{tab:fv}
\end{table*}


==> futurework.tex <==
\section{Conclusions and future directions}


==> preprocessing.tex <==
\section{Preprocessing} \label{sec:pre}

\myboldunderline{Pose refinement:}
%While we will design our algorithm to be robust against camera pose
%errors, it is nonetheless important to make the pose as accurate as
%possible given the input RGBD stream.
Appearance cues will be unreliable for visual feature based camera
tracking at the presence of displays with dynamic visual contents. We
will use depthmaps to refine camera extrinsic parameters (i.e., rotation
and translation).
%
For every pair of adjacent depth frames, we use Iterative Closest
Point algorithm (ICP)~\cite{besl1992method} to update point correspondences and
the relative camera motion. We then set up a non-linear least squares
problem that updates the rotation and translation of all the
cameras. The problem minimizes the sum of squared distances of the
point correspondences obtained by ICP for each adjacent depth frame.
We solve the problem by Ceres~\cite{ceres-solver}.

%% Our experiments showed that the camera pose from Tango often contain
%% large errors, nearly $X$ pixels in the image domain, especially in close
%% proximity to the display with dynamic apperance. \yasu{Hang, fill in X}
%% This step generally reduces the amount of reprojection errors to $Y$
%% pixels.

\myboldunderline{Depthmap reinforcement:} The depthmap resolution
($320\times 180$) is four times lower than the image resolution
($1280\times 720$). We will densify each depthmap by simply projecting
all the other 3D points. More precisely, we project each 3D point
into all the other frames and keep the minimum depth at each pixel. Note
that we simply associate a depth value to the closest pixel in each
frame, instead of ``splat''~\cite{qsplat} depth values. This may
potentially create gaps in depthmaps and cause ``see-through'' effects
for far surfaces. However, we have not observed this issue in our
experiments and chosen this simple approach.
 
\myboldunderline{Line detection:} Line detection is the key to
effectively extract rectangular regions in images. We use LSD in
OpenCV~\cite{von2008lsd} to detect line segments in each image.  In
our datasets, the tablet is always in a landscape orientation, and
vertical lines are also vertical in the images. Therefore, we first
simply collect lines that are within 20 degrees from the image Y-axis
to form a vertical line cluster. In general, one can just use the
camera rotation information to correct the expected line direction.
%
Remaining line segments are also clustered via standard vanishing point
analysis~\cite{tardif2009non,toldo2008robust}.



% To simplify post processings, we first extract verticle lines in the
% scene. In our dataset, the camera is roughly in landscape position, so
% we simply extract lines within 20 degrees against Y axis of image as
% verticle cluster. For the dataset where the camera is not in landscape
% position, we can easily compensate the rotation by camera pose.

%
% Von Gioi, R. Grompone, et al. LSD: A fast line segment detector with a
% false detection control, IEEE Transactions on Pattern Analysis and
% Machine Intelligence 32.4 (2010): 722-732.
%
%

